Molecular Clouds Associated with {H \small{II}} regions and Candidates within l = 106.65$^\circ$ to 109.50$^\circ$ and b = ${-}$1.85$^\circ$ to 0.95$^\circ$

We present a large-scale simultaneous survey of the CO isotopologues ($\rm {}^{12}{CO}$, $\rm{}^{13}{CO}$, and $\rm{C}{}^{18}{O}$) J = 1 ${-}$ 0 line emission toward the Galactic plane region of l = 106.65$^\circ$ to 109.50$^\circ$ and b = ${-}$1.85$^\circ$ to 0.95$^\circ$ using the Purple Mountain Observatory 13.7 m millimeter-wavelength telescope. Except for the molecular gas in the solar neighborhood, the emission from the molecular gas in this region is concentrated in the velocity range of [${-}$60, ${-}$35] $\rm km~s^{-1}$. The gas in the region can be divided into four clouds, with mass in the range of $\sim$10$^{3}$ to 10$^{4}$\,${M_{\sun}}$. We have identified 25 filaments based on the $\rm {}^{13}{CO}$ data. The median excitation temperature, length, line mass, line width, and virial parameter of the filaments are 10.89 K, 8.49 pc, 146.11 ${M}_{\odot}~ \rm pc^{-1}$, 1.01 $\rm km~s^{-1}$, and 3.14, respectively. Among these filaments, eight have virial parameters of less than 2, suggesting that they are gravitationally bound and can lead to star formation. Nineteen {H \small {II}} regions or candidates have previously been found in the region and we investigate the relationships between these {H \small {II}} regions/candidates and surrounding molecular clouds in detail. Using morphology similarity and radial velocity consistency between {H \small {II}} regions/candidates and molecular clouds as evidence for association, and raised temperature and velocity broadening as signatures of interaction, we propose that 12 {H \small {II}} regions/candidates are associated with their surrounding molecular clouds. In the case of the {H \small {II}} region of S142, the energy of the {H \small {II}} region is sufficient to maintain the turbulence in the surrounding molecular gas.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

